OccamNets: Mitigating Dataset Bias by Favoring Simpler Hypotheses

Dataset bias and spurious correlations can significantly impair generalization in deep neural networks. Many prior efforts have addressed this problem using either alternative loss functions or sampling strategies that focus on rare patterns. We propose a new direction: modifying the network architecture to impose inductive biases that make the network robust to dataset bias. Specifically, we propose OccamNets, which are biased to favor simpler solutions by design. OccamNets have two inductive biases. First, they are biased to use as little network depth as needed for an individual example. Second, they are biased toward using fewer image locations for prediction. While OccamNets are biased toward simpler hypotheses, they can learn more complex hypotheses if necessary. In experiments, OccamNets outperform or rival state-of-the-art methods run on architectures that do not incorporate these inductive biases. Furthermore, we demonstrate that when the state-of-the-art debiasing methods are combined with OccamNets results further improve.

==> old/occam-networks-old.tex <==

\section{\gls*{OccamNets} for Image Classification }

%We consider the task of image classification on biased vision datasets for our work, where the goal is to learn a function $f: X \longrightarrow Y$, to predict the category $y \in Y$ of image $x \in X$. Input $x$ consists of signal $s$ that a system should ideally use to predict $y$, but also contains biases $b$, which are spuriously correlated with $y$. We hypothesize that applying Occam's principles i.e., enabling the networks to learn simpler solutions can help deal with such spurious correlations. To test this hypothesis, we propose convolutional neural networks that prefer using minimal required network depth and visual regions. \kk{This paragraph is also repeated a bit; esp the first half seems unnecessary; I would just say that: "In this section, we describe OccamNet, which tests our hypothesis that applying Occam's principle, i.e., ..... OccamNet is designed with two inductive biases that help achieve this goal; 1) Use only the blah blah...}



% \begin{figure}[ht]
%  \centering
%     \includegraphics[width=0.9\linewidth]{figures/network.jpg}
%       \caption{\gls*{OccamNets} \kk{Let me know if you need help with this diagram -- I'm assuming this is just a placeholder; If its not, it needs to be a bit better than now -- the components are there but needs more polish...}}
%       %\rs{I really appreciate the help! The link is in the comment right below (and also present at the top of the page). Would be nice to show easy vs difficult samples/may CAMs.}
%       \label{fig: network}
%       %https://app.diagrams.net/#G1aBQp0ng-oMfmCQTVIOcns93x5u13b2Gx
% \end{figure}


%\kk{If we're writing limited work section, we should talk about how we're just following what is commonly done in literature and limiting to CNNs, but we could also test on ViTs and other vision models, and this is a weakness.}\rs{Transformers are mentioned in the discussions section}

%\kk{Not all of them -- why not say they contain modules, with many networks, such as resnet or densenet containing modules..}\rs{Added densenet/resnet as examples.}
\rs{Yet to check for consistent usage of symbols...}

\kk{I went through the whole writeup; Here is how I would suggest to organize -- these are based on my comments below}


\kk{************************************************************}\\
\kk{START ORGANIZATION NOTES}\\
\kk{************************************************************}


\subsection{OccamNet Design}
\kk{This is where you would explain the main model diagram and how they fit together and introduce basic notations -- Lots of text from the "inductive bias" as well as a fair amount from sections on Training the exits, Training the gates and Supressing the CAM should go here...Here is a crude sample...}

We enable OccamNet to exit early and only use visual regions by the help of attaching exit modules (\kk{Need some name for the whole thing, I'll call it name 1}) to various stages of a traditional convolutional neural networks. Many CNNs such as ResNets consist of blocks which are natural points to attach our exit modules. Below we describe different components and their roles that allow us to achive our desired properties. The details about how they are trained is discussed in the next section.

Within each exit module, we have the following components, that serve different roles. The details


\textbf{A. }Constrained Region Selection Module (Needs another name here, call name2) : Consists of a shallow two-layer CNN followed by 1x1 Conv. Epre blah blah blah. unit that produces a CAM. The CA maps are trained, via the CAM Supression Loss such that only a few regions provide informative signal about the ground truth class. ($\lambda_{CS}$, described in the next section..)


\textbf{B.} Exits (needs another name, such as Intermediate output or Exit Node, call it name3 ): Each exit node only receives a small subset of the image regions via Region selection module and serves as a self-contained answering/classification unit that is capable of producing the final prediction. The predictions are made using blah blah blah $\hat{y}$ blah blah blah. Each exit nodes is trained with a regular CE loss between $\hat{y}, y$, but these CE losses are modulated such that earlier nodes favor easier samples and latter nodes favor those that are missed by earlier nodes. This is achieved via the output loss ($\lambda_{O}$, described in the next section..) which is a weighted sum of CE losses attached to each node.  \rs{Calling this output predictor, which is basically just global average pooling on the CAMs predicted by the previous CAM predictor module. We can probably just focus on how this is obtained and what this is used for rather than treating this as a separate module. Also, need to foreshadow the exit gates since they are used to weigh the losses of 'exit nodes'/'output predictors'.}

\kk{Actually is the output loss really summed, it looks like there are several losses all backpropagating different lenghts of network. I am sure it is implemented as a sum in pytorch but is it thematically correct to call it a sum or just a series of N losses?}. \rs{The exit gate losses are completely detached (did better in the preliminary expts.). The CAM suppression losses and output CE losses are detached only for the first exit (so that features in general are good).}

\textbf{C. }Exit Gates (maybe also needs a new name but this one is fine as is. Some other options are Exit Decision Gate, Exit Switch?); Each exit node will produce its own copy of predictions. However, we still need to decide which nodes decision to trust during inference. This is done by training exit gates, which is attached to blah blah blah.


Taken together, the whole Occam network is trained via unified Occam Loss as follows:

\kk{INSERT LOSS FIGURE HERE}


Next, we describe how each of these losses are trained to control the desired inductive biases in our network.

\subsection{Training OccamNet}

\kk{This subsection should now just start with the hard details, no backstory, just maths...I'll outline some notes again}

\textbf{Training the Supression of CAMs}
By default, CAMs produce a NxN cells of outputs with each region containing confidence maps for different classes. We train the CAM maps to be peaky by blah blah cyhat, CS loss all that stuff.

\textbf{Training Exit Nodes (name3)}: Exit Nodes produce $\hat{y}$ by blah blah. Rest of this is mostly just "Training the Exits Section" as it is right now, minus some backstory

\textbf{Training Exit Gates}: For a given sample during inference, the output of exit gate, Gj is used to decide whether to terminate or not blah blah 0.5 blah blah. To trainj we use, blah blah blah \kk{Copy rest of the "training the exit gates" section mostly}


\kk{************************************************************}\\
\kk{END ORGANIZATION NOTES}\\
\kk{************************************************************}


\subsection{Proposed Inductive Biases}
Commonly used convolutional neural networks (CNNs) such as ResNets~\cite{he2016deep} and DenseNets~\cite{huang2017densely} consist of a sequence of modules $M(.)$, each of which contains one or more convolutional layers. Usually, the final feature maps are collected through global average pooling and fed into a linear classifier to obtain the predictions. \gls*{OccamNets} add two inductive biases to this conventional setup to improve bias robustness:

\textbf{Inductive Bias \#1: Favor Shallower Network Depths.} The first inductive bias encourages the samples to exit as early as possible, with deeper layers being used \kk{only} for samples that the earlier layers fail to classify correctly. For this, \gls*{OccamNets} attach intermediate exits $E_j(.)$ and exit gating networks $G_j(.)$ to the intermediate convolutional modules $M_j(.)$. Here, each exit $E_j(.)$ outputs its predictions: $\hat{y} = E(.)$ and is trained with the output loss $\mathcal{L}_O$. The exit gating network, $G$ decides whether or not to terminate the computation at depth $j$ for each sample by yielding an exit probability score $\hat{g}$. $G(.)$ is trained with an exit gating loss, $\mathcal{L}_{G}$, which is described in Sec.~\ref{sec:exits} \kk{What is the purpose of just name dropping this loss right now? Either just talk about it now, or remove this line. Or third option, at least describe what this controls/does}. To encourage a deeper module $M_j$, to focus on samples that the earlier module $M_{j-1}$ finds difficult, we use $\hat{g}_{j-1}$ to weigh $E_j$'s loss $\mathcal{L}_{O,j}$.

\textbf{Inductive Bias \#2: Favor Fewer Visual Regions.} The second inductive bias is to favor using a constrained set of regions instead of using all the visual regions. For this, \gls*{OccamNets} use exits that yield class activation maps (CAMs) that are trained to rely on fewer visual regions. Specifically, each exit consists only of convolutional layers to output spatial maps, that are trained with CAM suppression loss ($\mathcal{L}_{CS}$) that encourages only a few regions to affect the predictions. The details are provided in Sec.~\ref{sec:cams}. \kk{Again, same as above, what is the purpose of just name dropping this loss right now? Either just talk about it now, or remove this line. Or third option, at least describe what this controls/does}

Denoting loss weights by $\lambda$, the total loss used to train \gls*{OccamNets} is thus given by:

\begin{figure}[h!]
 \centering
 \vspace{-0.8cm}
    \includegraphics[width=0.9\linewidth]{figures/losses.jpg}
      \caption{Losses for \gls*{OccamNets}}
      \label{fig:losses}
\end{figure}

%We first describe how we train the network to exit as early as possible ($\mathcal{L_{E}}+ \mathcal{L_{G}}$) in Sec.~\ref{sec:early_exits}, and then describe our training mechanism for the exits that produce constrained class activation maps ($\mathcal{L_{CAM}}$) in Sec.~\ref{sec:cams}.

%\kk{I suggested a way to do this; I think the equation should be annotated further for clarity; I could do that if we decided to go this way. In any case, I think we should give each of our three losses some names and maybe change acronyms accordingly. E.g., Output Loss: Lo, exit control loss Lec, and region confidence Lrc or region supression loss Lls. In other words, based on what they do rather than what they are maybe??}\rs{Addressed}

\textbf{Exit Components.}
\kk{We have already had to describe function of exit much earlier -- it seems too late to talk about it just now...}
Each exit $E$ consists of a pre-exit module $E_{pre}(.)$ that produces intermediate representations that are fed into CAM module $E_{C}$ and exit gating module $G$. CAM module $E_{C}$ produces a class activation map $c \in \mathbb{R}^{h \times w \times n_Y}$ where $h$ and $w$ are the height and width of the map and $n_Y$ is the total number of classes. Each cell in the map provides a softmax score for each of the classes. To obtain classwise prediction scores, we apply global average pooling on the CAMs. Pre-exit module, $E_{pre}$ consists of two $3 \times $3 convolutional layers and $E_{C}$ consists of single $1 \times 1$ convolutional layer. Furthermore, each exit is also associated with an exit gating network $G$, realized via a ReLU layer followed by a sigmoid layer. \kk{None of this is clear -- instead of just technical details please go into what they do in contef exiting the network or producing CAM maps..}

We now first describe how the exit gates are trained (Sec.~\ref{sec:exit_gates}) and then describe how their outputs are used to train the main exits (Sec.~\ref{sec:exits}). Then in Sec.~\ref{sec:cams} we describe the constrained CAMs.
 
\subsection{Training the Exit Gates}
\label{sec:exit_gates}
Exit gate $G_j(.)$ decides whether or not a sample should exit by yielding an exit probability score $\hat{g_j} = G_j(.)$, where, $\hat{g_j} \ge 0.5$ indicates that the sample can exit from $E_j$ and $\hat{g}_j < 0.5$ indicates that the sample must continue to the next module $M_{j+1}$. Hard exit is performed only during inference. $G_j$ is trained with the gating loss:
\begin{align}
\mathcal{L}_G = \sum_{k \in \{0,1\}} \frac{\mathbbm{1}(g_j=k) BCE(g_j, \hat{g_j})}{\sqrt{\sum \mathbbm{1}(g_j=k)}},
\end{align}
where $g_j$ is the ground truth value for the $j^{th}$ gate:
\begin{align}
    g_j = 
\begin{cases}
    1,& \text{if } \hat{y_j} = y  \\
    0,              & \text{otherwise},
\end{cases}
\end{align} 
i.e., $G_j$ is trained to exit if the sample is correctly predicted, else it is trained to continue onto the next module.  Furthermore, we balance out the contributions from the samples with $g=1$ and $g=0$ to avoid biasing one decision over the other. With this setup, sufficiently parameterized models that obtain $100\%$ training accuracy will result in a trivial solution where $g_j$ is always set to $1$ i.e., the exit will learn that all the samples can exit. To avoid this issue, we stop computing $g_j$ once $E_j$'s training accuracy reaches a predefined threshold $\tau_{acc,j}$. During training, the gradients from $G$ do not train $E_{pre}(.)$ or $M(.)$.%During inference, samples with $\hat{g_j} > 0.5$ exit from $E_j$. 
 
\subsection{Training the Exits}
\label{sec:exits}
We train the exits with a loss weighting scheme that encourages the earliest exit to focus on bias-prone/easy samples, thereby, helping the later exits to focus on bias-conflicting/difficult samples. Specifically, we train a bias-amplified first exit $E_0$, using the following loss weight:
\begin{align}
    \mathcal{W}_0 = p_0^{\gamma_0},
\end{align}
where, $p_0$ is the softmax score for the ground truth class predicted by $E_0$ and $\gamma_0 > 0$ encourages $E_0$ to focus on easier samples. We set $\gamma_0 = 3$ to sufficiently amplify biases in all the experiments \kk{This is not clear, clearly explain why scaling the probabalities by a positive factor means that they will be easier. ALso, what does loss weight mean?? Why is W0 not a part of eqn 5? Why is W0 not flowing through the netowrk M? Several things are unclear here}. The subsequent exits are then encouraged to focus on samples that the preceding exits find difficult. For this, the loss weights are defined as:
\begin{align}
    \mathcal{W}_j = (1 - g_{j-1} + \epsilon),~\text{if j  $>$ 0},
\end{align}

where, $g_{j-1}$ is the exit score predicted by $(j-1)^{th}$ exit gate and $\epsilon=0.1$ is a small offset to ensure that all the samples receive a minimal loss weight. For the samples where $G_{j-1}$ is not confident, the weight loss for $j^{th}$ exit, $\mathcal{W}_j$ becomes high. The total output loss is then:
\begin{align}
    \mathcal{L}_O = \sum_{j=1}^{n_E} \mathcal{W}_j ~ CE(\hat{y}_j, y),
\end{align}
where, $CE(\hat{y}_j, y)$ is the cross-entropy loss between $E_j$'s prediction $\hat{y}_j$ obtained after performing global average pooling on the CAM and the ground truth label $y$ and $n_E$ is the total number of exits.

During training, we prevent the gradients of the first, bias-amplified exit, $E_0$ from passing through $M(.)$.


\subsection{Suppressing the Class Activation Maps}
\label{sec:cams}
Next we describe how the model is encouraged to constrain the usage of visual regions. For this, we regularize the maps \kk{How are these maps generated; that information is way too far from here --} such that only some of the cells exhibit confidence towards the ground truth class, whereas rest of the cells exhibit inconfidence i.e., have uniform prediction scores for all the classes. Specifically, let $c_y \in \mathbb{R}^{h \times w}$ be the class activation map for the ground truth class. Then, we apply regularization on the cells that obtain softmax scores lower than the average softmax score for the ground truth class. That is, let $\overline{c}_y$ be the softmax score averaged over all the cells in $c_y$, then a cell at location $l$, $c^l \in \mathbb{R}^{n_Y}$ is regularized if its softmax score for the ground truth class, $c^l_y$ is less than $\overline{c}_y$. The CAM suppression loss is given below:
\begin{align}
    \mathcal{L}_{CS} = \sum_{l=1}^{hw} \mathbbm{1} (c_y^l < \overline{c}_y) ~KLD(c^l, \frac{1}{n_Y}\mathbf{1}),
\end{align}
where, $KLD(c^l, \frac{1}{n_Y}\mathbf{1})$ is the KL-divergence loss with respect to a uniform class distribution and $\mathbbm{1} (c_y^l < \overline{c}_y)$ ensures that the loss is applied only on the cells with scores lower than $\overline{c}_y$.




%The first inductive bias in \gls*{OccamNets} encourages the network to exit from shallower network layers whenever appropriate. During training, deeper layers focus on samples that the shallower layers fail to classify correctly. At inference-time, this enables the network to dynamically choose processing depth for each sample.

%Intuitively, shallower layers should suffice for easier \kk{Again, what is easy, consider rephrasing} samples, and that would enable the later layers to focus on more difficult \kk{Easy and difficult are still not well defined} samples. The underlying hypothesis is that a network that can dynamically choose the processing depth \kk{for a given sample} thus has the ability to generalize to both easy and difficult samples.

%\kk{I don't understand the difference between learning to exit vs training the exit -- I mean I understand how they work, but dont understand the name choice or the decision to organize it like this. I think we should say as: OccamNet has multiple outputs, each of which is trained with BCE loss; To choose where to exit we use the Lg; In a single paragraph. Then, I would put the multiple output layers before this subheader. that is before "Inductive bias 1". (Yes, we will need to modify the loss figure as well if we do this). Then, we can start this subsection with "Having the output at different depth allows networks to make predictions at various depths. Now, we train the network so that it chooses to exit early (take output from earlier output layers) for easier samples and vice-versa for difficult samples. (I'm using easy/difficult to keep with what you've been saying but I don't think this is a good terminology without proper definition somewhere above.).... }

% The total loss is given by:
% \begin{align}
%     \mathcal{L}_{Occam} = \mathcal{L}_E + \lambda_G \mathcal{L}_G + \lambda_{CAM} \mathcal{L}_{CAM},
% \end{align}
% where, $\lambda_G$ is set to 1 and $\lambda_{CAM}$ is set to 0.1 for all of the experiments. \ck{move to the top of section 3, it doesn't really go here, and you could then say what each loss does and how you will explain them in greater detail in dedicated sections}

%\kk{The technical presentation is pretty clear and sufficient but the organization could use some work: It is unclear why the output loss Le is lumped with inductive bias number 1 -- I sorta see why but I am not sure if that is the best way. I also agree with putting total loss up-top. Alternatively, we would need to get creative on how to give the big picture first visually.}\rs{The main loss is weighted using outputs from the exit gates i.e., deeper layers are trained to focus on samples that earlier layers found difficult. Gates and exits are kind of tied together in that regards. Need to make it clearer.}

%\subsection{Implementation Details}
%\textbf{Exits and Gates.}


%\textbf{Occam ResNets.}
%For all of our experiments, we build upon the ResNet architecture~\cite{he2016deep}. ResNets consist of four modules/sub-models, each of which has several residual convolutional blocks. We place exits and exit gates at the end of each of those modules. We further constrain the number of parameters by reducing the feature width to 48 instead of the commonly used value of 64. In Table~\ref{tab:arch-comparison}, we compare the intermediate modules, exit/gating modules and the number of trainable parameters for Standard vs. Occam ResNet architectures.
%\input{tables/arch-comparison}

%\kk{I am not fully sure how, but this organization is a bit weird. Shouldn't the implementation of exits and pre-exits described before the losses? Wouldn't the Occam Resnet better belong at the "Model overview" paragraph above -- we already talk about CNNs and modules there, why not just discuss resnet there? I understand the need to generic --> specific but I think that point could be made in a more streamlined way; Right now the information is fragmented unnecessarily -- when in reality it is quite simple. For different points in Resnet, we attach these exit gates (pre-exit module + CAM module), attach Le to each of these to predict output, Then, Lg and Lcam modulate when to exit (which output to use) and which regions to use. This mental picture should be clear to readers without too much effort -- RIght now, I think it is a bit hard.}

==> old/occam-networks-with-Kushal-comments.tex <==

\section{\gls*{OccamNets} for Image Classification }

We consider the task of image classification on biased vision datasets for our work, where the goal is to learn a function $f: X \longrightarrow Y$, to predict the category $y \in Y$ of image $x \in X$. Input $x$ consists of signal $s$ that a system should ideally use to predict $y$, but also contains biases $b$, which are spuriously correlated with $y$. We hypothesize that applying Occam's principles i.e., enabling the networks to learn simpler solutions can help deal with such spurious correlations. To test this hypothesis, we propose convolutional neural networks that prefer using minimal required network depth and visual regions. \kk{This paragraph is also repeated a bit; esp the first half seems unnecessary; I would just say that: "In this section, we describe OccamNet, which tests our hypothesis that applying Occam's principle, i.e., ..... OccamNet is designed with two inductive biases that help achieve this goal; 1) Use only the blah blah...}



\begin{figure}[ht]
 \centering
    \includegraphics[width=0.9\linewidth]{figures/network.jpg}
      \caption{\gls*{OccamNets} \kk{Let me know if you need help with this diagram -- I'm assuming this is just a placeholder; If its not, it needs to be a bit better than now -- the components are there but needs more polish...}}
      %\rs{I really appreciate the help! The link is in the comment right below (and also present at the top of the page). Would be nice to show easy vs difficult samples/may CAMs.}
      \label{fig: network}
      %https://app.diagrams.net/#G1aBQp0ng-oMfmCQTVIOcns93x5u13b2Gx
\end{figure}


%\kk{If we're writing limited work section, we should talk about how we're just following what is commonly done in literature and limiting to CNNs, but we could also test on ViTs and other vision models, and this is a weakness.}\rs{Transformers are mentioned in the discussions section}

%\kk{Not all of them -- why not say they contain modules, with many networks, such as resnet or densenet containing modules..}\rs{Added densenet/resnet as examples.}
\rs{Yet to check for consistent usage of symbols...}

\kk{I went through the whole writeup; Here is how I would suggest to organize -- these are based on my comments below}


\kk{************************************************************}\\
\kk{START ORGANIZATION NOTES}\\
\kk{************************************************************}


\subsection{OccamNet Design}
\kk{This is where you would explain the main model diagram and how they fit together and introduce basic notations -- Lots of text from the "inductive bias" as well as a fair amount from sections on Training the exits, Training the gates and Supressing the CAM should go here...Here is a crude sample...}

We enable OccamNet to exit early and only use visual regions by the help of attaching exit modules (\kk{Need some name for the whole thing, I'll call it name 1}) to various stages of a traditional convolutional neural networks. Many CNNs such as ResNets consist of blocks which are natural points to attach our exit modules. Below we describe different components and their roles that allow us to achive our desired properties. The details about how they are trained is discussed in the next section.

Within each exit module, we have the following components, that serve different roles. The details


\textbf{A. }Constrained Region Selection Module (Needs another name here, call name2) : Consists of a shallow two-layer CNN followed by 1x1 Conv. Epre blah blah blah. unit that produces a CAM. The CA maps are trained, via the CAM Supression Loss such that only a few regions provide informative signal about the ground truth class. ($\lambda_{CS}$, described in the next section..)


\textbf{B.} Exits (needs another name, such as Intermediate output or Exit Node, call it name3 ): Each exit node only receives a small subset of the image regions via Region selection module and serves as a self-contained answering/classification unit that is capable of producing the final prediction. The predictions are made using blah blah blah $\hat{y}$ blah blah blah. Each exit nodes is trained with a regular CE loss between $\hat{y}, y$, but these CE losses are modulated such that earlier nodes favor easier samples and latter nodes favor those that are missed by earlier nodes. This is achieved via the output loss ($\lambda_{O}$, described in the next section..) which is a weighted sum of CE losses attached to each node.  \rs{Exits encapulate 'constrained region selection module' though. n fact output of exit is CAMs.}

\kk{Actually is the output loss really summed, it looks like there are several losses all backpropagating different lenghts of network. I am sure it is implemented as a sum in pytorch but is it thematically correct to call it a sum or just a series of N losses?}. 

\textbf{C. }Exit Gates (maybe also needs a new name but this one is fine as is. Some other options are Exit Decision Gate, Exit Switch?); Each exit node will produce its own copy of predictions. However, we still need to decide which nodes decision to trust during inference. This is done by training exit gates, which is attached to blah blah blah.


Taken together, the whole Occam network is trained via unified Occam Loss as follows:

\kk{INSERT LOSS FIGURE HERE}


Next, we describe how each of these losses are trained to control the desired inductive biases in our network.

\subsection{Training OccamNet}

\kk{This subsection should now just start with the hard details, no backstory, just maths...I'll outline some notes again}

\textbf{Training the Supression of CAMs}
By default, CAMs produce a NxN cells of outputs with each region containing confidence maps for different classes. We train the CAM maps to be peaky by blah blah cyhat, CS loss all that stuff.

\textbf{Training Exit Nodes (name3)}: Exit Nodes produce $\hat{y}$ by blah blah. Rest of this is mostly just "Training the Exits Section" as it is right now, minus some backstory

\textbf{Training Exit Gates}: For a given sample during inference, the output of exit gate, Gj is used to decide whether to terminate or not blah blah 0.5 blah blah. To trainj we use, blah blah blah \kk{Copy rest of the "training the exit gates" section mostly}


\kk{************************************************************}\\
\kk{END ORGANIZATION NOTES}\\
\kk{************************************************************}


\subsection{Proposed Inductive Biases}
Commonly used convolutional neural networks (CNNs) such as ResNets~\cite{he2016deep} and DenseNets~\cite{huang2017densely} consist of a sequence of modules $M(.)$, each of which contains one or more convolutional layers. Usually, the final feature maps are collected through global average pooling and fed into a linear classifier to obtain the predictions. \gls*{OccamNets} add two inductive biases to this conventional setup to improve bias robustness:

\textbf{Inductive Bias \#1: Favor Shallower Network Depths.} The first inductive bias encourages the samples to exit as early as possible, with deeper layers being used \kk{only} for samples that the earlier layers fail to classify correctly. For this, \gls*{OccamNets} attach intermediate exits $E_j(.)$ and exit gating networks $G_j(.)$ to the intermediate convolutional modules $M_j(.)$. Here, each exit $E_j(.)$ outputs its predictions: $\hat{y} = E(.)$ and is trained with the output loss $\mathcal{L}_O$. The exit gating network, $G$ decides whether or not to terminate the computation at depth $j$ for each sample by yielding an exit probability score $\hat{g}$. $G(.)$ is trained with an exit gating loss, $\mathcal{L}_{G}$, which is described in Sec.~\ref{sec:exits} \kk{What is the purpose of just name dropping this loss right now? Either just talk about it now, or remove this line. Or third option, at least describe what this controls/does}. To encourage a deeper module $M_j$, to focus on samples that the earlier module $M_{j-1}$ finds difficult, we use $\hat{g}_{j-1}$ to weigh $E_j$'s loss $\mathcal{L}_{O,j}$.

\textbf{Inductive Bias \#2: Favor Fewer Visual Regions.} The second inductive bias is to favor using a constrained set of regions instead of using all the visual regions. For this, \gls*{OccamNets} use exits that yield class activation maps (CAMs) that are trained to rely on fewer visual regions. Specifically, each exit consists only of convolutional layers to output spatial maps, that are trained with CAM suppression loss ($\mathcal{L}_{CS}$) that encourages only a few regions to affect the predictions. The details are provided in Sec.~\ref{sec:cams}. \kk{Again, same as above, what is the purpose of just name dropping this loss right now? Either just talk about it now, or remove this line. Or third option, at least describe what this controls/does}

Denoting loss weights by $\lambda$, the total loss used to train \gls*{OccamNets} is thus given by:

\begin{figure}[h!]
 \centering
 \vspace{-0.8cm}
    \includegraphics[width=0.9\linewidth]{figures/losses.jpg}
      \caption{Losses for \gls*{OccamNets}}
      \label{fig: network}
\end{figure}

%We first describe how we train the network to exit as early as possible ($\mathcal{L_{E}}+ \mathcal{L_{G}}$) in Sec.~\ref{sec:early_exits}, and then describe our training mechanism for the exits that produce constrained class activation maps ($\mathcal{L_{CAM}}$) in Sec.~\ref{sec:cams}.

%\kk{I suggested a way to do this; I think the equation should be annotated further for clarity; I could do that if we decided to go this way. In any case, I think we should give each of our three losses some names and maybe change acronyms accordingly. E.g., Output Loss: Lo, exit control loss Lec, and region confidence Lrc or region supression loss Lls. In other words, based on what they do rather than what they are maybe??}\rs{Addressed}

\textbf{Exit Components.}
\kk{We have already had to describe function of exit much earlier -- it seems too late to talk about it just now...}
Each exit $E$ consists of a pre-exit module $E_{pre}(.)$ that produces intermediate representations that are fed into CAM module $E_{C}$ and exit gating module $G$. CAM module $E_{C}$ produces a class activation map $c \in \mathbb{R}^{h \times w \times n_Y}$ where $h$ and $w$ are the height and width of the map and $n_Y$ is the total number of classes. Each cell in the map provides a softmax score for each of the classes. To obtain classwise prediction scores, we apply global average pooling on the CAMs. Pre-exit module, $E_{pre}$ consists of two $3 \times $3 convolutional layers and $E_{C}$ consists of single $1 \times 1$ convolutional layer. Furthermore, each exit is also associated with an exit gating network $G$, realized via a ReLU layer followed by a sigmoid layer. \kk{None of this is clear -- instead of just technical details please go into what they do in contef exiting the network or producing CAM maps..}

We now first describe how the exit gates are trained (Sec.~\ref{sec:exit_gates}) and then describe how their outputs are used to train the main exits (Sec.~\ref{sec:exits}). Then in Sec.~\ref{sec:cams} we describe the constrained CAMs.
 
\subsection{Training the Exit Gates}
\label{sec:exit_gates}
Exit gate $G_j(.)$ decides whether or not a sample should exit by yielding an exit probability score $\hat{g_j} = G_j(.)$, where, $\hat{g_j} \ge 0.5$ indicates that the sample can exit from $E_j$ and $\hat{g}_j < 0.5$ indicates that the sample must continue to the next module $M_{j+1}$. Hard exit is performed only during inference. $G_j$ is trained with the gating loss:
\begin{align}
\mathcal{L}_G = \sum_{k \in \{0,1\}} \frac{\mathbbm{1}(g_j=k) BCE(g_j, \hat{g_j})}{\sqrt{\sum \mathbbm{1}(g_j=k)}},
\end{align}
where $g_j$ is the ground truth value for the $j^{th}$ gate:
\begin{align}
    g_j = 
\begin{cases}
    1,& \text{if } \hat{y_j} = y  \\
    0,              & \text{otherwise},
\end{cases}
\end{align} 
i.e., $G_j$ is trained to exit if the sample is correctly predicted, else it is trained to continue onto the next module.  Furthermore, we balance out the contributions from the samples with $g=1$ and $g=0$ to avoid biasing one decision over the other. With this setup, sufficiently parameterized models that obtain $100\%$ training accuracy will result in a trivial solution where $g_j$ is always set to $1$ i.e., the exit will learn that all the samples can exit. To avoid this issue, we stop computing $g_j$ once $E_j$'s training accuracy reaches a predefined threshold $\tau_{acc,j}$. During training, the gradients from $G$ do not train $E_{pre}(.)$ or $M(.)$.%During inference, samples with $\hat{g_j} > 0.5$ exit from $E_j$. 
 
\subsection{Training the Exits}
\label{sec:exits}
We train the exits with a loss weighting scheme that encourages the earliest exit to focus on bias-prone/easy samples, thereby, helping the later exits to focus on bias-conflicting/difficult samples. Specifically, we train a bias-amplified first exit $E_0$, using the following loss weight:
\begin{align}
    \mathcal{W}_0 = p_0^{\gamma_0},
\end{align}
where, $p_0$ is the softmax score for the ground truth class predicted by $E_0$ and $\gamma_0 > 0$ encourages $E_0$ to focus on easier samples. We set $\gamma_0 = 3$ to sufficiently amplify biases in all the experiments \kk{This is not clear, clearly explain why scaling the probabalities by a positive factor means that they will be easier. ALso, what does loss weight mean?? Why is W0 not a part of eqn 5? Why is W0 not flowing through the netowrk M? Several things are unclear here}. The subsequent exits are then encouraged to focus on samples that the preceding exits find difficult. For this, the loss weights are defined as:
\begin{align}
    \mathcal{W}_j = (1 - g_{j-1} + \epsilon),~\text{if j  $>$ 0},
\end{align}

where, $g_{j-1}$ is the exit score predicted by $(j-1)^{th}$ exit gate and $\epsilon=0.1$ is a small offset to ensure that all the samples receive a minimal loss weight. For the samples where $G_{j-1}$ is not confident, the weight loss for $j^{th}$ exit, $\mathcal{W}_j$ becomes high. The total output loss is then:
\begin{align}
    \mathcal{L}_O = \sum_{j=1}^{n_E} \mathcal{W}_j ~ CE(\hat{y}_j, y),
\end{align}
where, $CE(\hat{y}_j, y)$ is the cross-entropy loss between $E_j$'s prediction $\hat{y}_j$ obtained after performing global average pooling on the CAM and the ground truth label $y$ and $n_E$ is the total number of exits.

During training, we prevent the gradients of the first, bias-amplified exit, $E_0$ from passing through $M(.)$.


\subsection{Suppressing the Class Activation Maps}
\label{sec:cams}
Next we describe how the model is encouraged to constrain the usage of visual regions. For this, we regularize the maps \kk{How are these maps generated; that information is way too far from here --} such that only some of the cells exhibit confidence towards the ground truth class, whereas rest of the cells exhibit inconfidence i.e., have uniform prediction scores for all the classes. Specifically, let $c_y \in \mathbb{R}^{h \times w}$ be the class activation map for the ground truth class. Then, we apply regularization on the cells that obtain softmax scores lower than the average softmax score for the ground truth class. That is, let $\overline{c}_y$ be the softmax score averaged over all the cells in $c_y$, then a cell at location $l$, $c^l \in \mathbb{R}^{n_Y}$ is regularized if its softmax score for the ground truth class, $c^l_y$ is less than $\overline{c}_y$. The CAM suppression loss is given below:
\begin{align}
    \mathcal{L}_{CS} = \sum_{l=1}^{hw} \mathbbm{1} (c_y^l < \overline{c}_y) ~KLD(c^l, \frac{1}{n_Y}\mathbf{1}),
\end{align}
where, $KLD(c^l, \frac{1}{n_Y}\mathbf{1})$ is the KL-divergence loss with respect to a uniform class distribution and $\mathbbm{1} (c_y^l < \overline{c}_y)$ ensures that the loss is applied only on the cells with scores lower than $\overline{c}_y$.




%The first inductive bias in \gls*{OccamNets} encourages the network to exit from shallower network layers whenever appropriate. During training, deeper layers focus on samples that the shallower layers fail to classify correctly. At inference-time, this enables the network to dynamically choose processing depth for each sample.

%Intuitively, shallower layers should suffice for easier \kk{Again, what is easy, consider rephrasing} samples, and that would enable the later layers to focus on more difficult \kk{Easy and difficult are still not well defined} samples. The underlying hypothesis is that a network that can dynamically choose the processing depth \kk{for a given sample} thus has the ability to generalize to both easy and difficult samples.

%\kk{I don't understand the difference between learning to exit vs training the exit -- I mean I understand how they work, but dont understand the name choice or the decision to organize it like this. I think we should say as: OccamNet has multiple outputs, each of which is trained with BCE loss; To choose where to exit we use the Lg; In a single paragraph. Then, I would put the multiple output layers before this subheader. that is before "Inductive bias 1". (Yes, we will need to modify the loss figure as well if we do this). Then, we can start this subsection with "Having the output at different depth allows networks to make predictions at various depths. Now, we train the network so that it chooses to exit early (take output from earlier output layers) for easier samples and vice-versa for difficult samples. (I'm using easy/difficult to keep with what you've been saying but I don't think this is a good terminology without proper definition somewhere above.).... }

% The total loss is given by:
% \begin{align}
%     \mathcal{L}_{Occam} = \mathcal{L}_E + \lambda_G \mathcal{L}_G + \lambda_{CAM} \mathcal{L}_{CAM},
% \end{align}
% where, $\lambda_G$ is set to 1 and $\lambda_{CAM}$ is set to 0.1 for all of the experiments. \ck{move to the top of section 3, it doesn't really go here, and you could then say what each loss does and how you will explain them in greater detail in dedicated sections}

%\kk{The technical presentation is pretty clear and sufficient but the organization could use some work: It is unclear why the output loss Le is lumped with inductive bias number 1 -- I sorta see why but I am not sure if that is the best way. I also agree with putting total loss up-top. Alternatively, we would need to get creative on how to give the big picture first visually.}\rs{The main loss is weighted using outputs from the exit gates i.e., deeper layers are trained to focus on samples that earlier layers found difficult. Gates and exits are kind of tied together in that regards. Need to make it clearer.}

%\subsection{Implementation Details}
%\textbf{Exits and Gates.}


%\textbf{Occam ResNets.}
%For all of our experiments, we build upon the ResNet architecture~\cite{he2016deep}. ResNets consist of four modules/sub-models, each of which has several residual convolutional blocks. We place exits and exit gates at the end of each of those modules. We further constrain the number of parameters by reducing the feature width to 48 instead of the commonly used value of 64. In Table~\ref{tab:arch-comparison}, we compare the intermediate modules, exit/gating modules and the number of trainable parameters for Standard vs. Occam ResNet architectures.
%\input{tables/arch-comparison}

%\kk{I am not fully sure how, but this organization is a bit weird. Shouldn't the implementation of exits and pre-exits described before the losses? Wouldn't the Occam Resnet better belong at the "Model overview" paragraph above -- we already talk about CNNs and modules there, why not just discuss resnet there? I understand the need to generic --> specific but I think that point could be made in a more streamlined way; Right now the information is fragmented unnecessarily -- when in reality it is quite simple. For different points in Resnet, we attach these exit gates (pre-exit module + CAM module), attach Le to each of these to predict output, Then, Lg and Lcam modulate when to exit (which output to use) and which regions to use. This mental picture should be clear to readers without too much effort -- RIght now, I think it is a bit hard.}

==> tables/arch-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Architecture Comparison \kk{If we write section 3 properly as Chris and I commented, I think this would be unnecessary.  In the main paper at least. We can just comment how our modification does not increase the number of parameters in text.}}
\label{tab:arch-comparison}
\addtolength\tabcolsep{3pt}
\begin{tabular}{lll}
 \hline
Components & Standard \gls*{ResNet} & \gls*{OccamResNet} \\ \hline
%Input block(s) & \begin{tabular}[l]{@{}l@{}}Single, learned block\end{tabular} & \begin{tabular}[l]{@{}l@{}}Fixed PCA weights \\ Separate input block \\ per module\end{tabular} \\ \hline
Intermediate modules & \begin{tabular}[l]{@{}l@{}}4 modules, each with \\ feature width=64\end{tabular} & \begin{tabular}[l]{@{}l@{}}4 modules, each with \\ feature width=48 \end{tabular} \\ \hline
Exit(s) & \begin{tabular}[l]{@{}l@{}}Single exit at the end with \\ global average pooling \\ and linear classifier\end{tabular} & \begin{tabular}[l]{@{}l@{}} One exit per module, \\ each predicting class\\ activation maps \end{tabular} \\ \hline
\# of parameters \\ e.g., ResNet18 & \begin{tabular}[l]{@{}c@{}} 11,689,512 \end{tabular} & \begin{tabular}[l]{@{}c@{}} 7,939,860 \end{tabular} \\ 
\hline

\end{tabular}%
\end{table}

==> tables/biased-mnist-averaged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Accuracies on majority (maj)/minority (min) groups for each bias variable in \gls*{BiasedMNIST} ($p_{bias}=0.95$), averaged over the comparison methods. We format the results with the lowest differences between the groups.}
\label{tab:biased-mnist}
\addtolength\tabcolsep{1.75pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc} \hline
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Variables/\\ Methods\end{tabular}}} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Scale\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit\\ Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture \\Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter \\ Color\end{tabular}} \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Test \\ Acc.\end{tabular}} &
  \multicolumn{2}{c}{maj/min} &
  \multicolumn{2}{c}{maj/min} &
  \multicolumn{2}{c}{maj/min} &
  \multicolumn{2}{c}{maj/min} &
  \multicolumn{2}{c}{maj/min} &
  \multicolumn{2}{c}{maj/min}
  \\ \hline
 \multicolumn{1}{l}{ResNet} &
  \multicolumn{1}{l}{40.1} &
  \multicolumn{2}{c}{87.6/34.8} &
  \multicolumn{2}{c}{80.2/28.5} &
  \multicolumn{2}{c}{76.9/35.9} &
  \multicolumn{2}{c}{44.4/39.6} &
  \multicolumn{2}{c}{52.2/38.7} &
  \multicolumn{2}{c}{49.3/39.1} \\
  \multicolumn{1}{l}{OccamResNet} &
  \multicolumn{1}{l}{63.9} &
  \multicolumn{2}{c}{94.4/60.5} &
  \multicolumn{2}{c}{95.6/60.3} &
  \multicolumn{2}{c}{82.9/61.7} &
  \multicolumn{2}{c}{\textbf{65.9/63.7}} &
  \multicolumn{2}{c}{\textbf{\underline{63.9/63.9}}} &
  \multicolumn{2}{c}{\textbf{\underline{63.9/63.9}}}
  \\ \hline

\end{tabular}}
\end{table*}

==> tables/celeba.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Results on \gls*{CelebA}}
\label{tab:celeba}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}c@{}}Non-Blond\\ Male\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Blond\\Male\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Non-Blond \\ Non-Male \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Blond \\ Non-Male\end{tabular}  &
  \begin{tabular}[c]{@{}c@{}}Mean Per \\ Group\end{tabular} \\ \hline
\multicolumn{6}{c}{\textit{ResNet-18 baselines}}                                                             \\
\gls*{ERM}  & 99.3 & 42.8 & 95.9 & 83.3 & 80.3 \\
\gls*{UpWt}   & 89.3 & 77.8 & 87.4 & 95.0 & 87.4 \\
\gls*{gDRO}~\cite{sagawa2019distributionally} & 91.2 & 80.0 & 90.9 & 92.1 & 88.5 \\
\gls*{PGI}~\cite{ahmed2020systematic}   & 98.2  & 63.3 & 96.5 & 83.9 & 85.5 \\
\gls*{SD}~\cite{pezeshki2020gradient}                                   & 96.4 & 73.3 & 88.0 & 96.6 & 88.6 \\
\hline
\multicolumn{6}{c}{\textit{OccamResNet-18 without Input Gating, Exit Gating and Dynamic Pooling}}                             \\
\gls*{ERM}               & & & & & \\
\gls*{UpWt}   & & & & & \\
\gls*{gDRO}~\cite{sagawa2019distributionally}   & & & & & \\
\gls*{PGI}~\cite{ahmed2020systematic}  & & & & & \\ 
\gls*{SD}~\cite{pezeshki2020gradient}     & & & & & \\\hline
\multicolumn{6}{c}{\textit{Ours: OccamResNet-18 with Input Gating, Exit Gating and Dynamic Pooling}}                                                 \\
OccamResNet-18                                                                            &  &  &  & &  \\ \hline
\end{tabular}%
\end{table}

==> tables/old/biased-mnist-3-sec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Unbiased Accuracy (i.e., overall test set accuracy) and Majority/Minority Accuracies per bias variable in \gls*{BiasedMNIST} ($p_{bias}=0.95$)}
\label{tab:biased-mnist}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc} \hline
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Variables/\\ Methods\end{tabular}}} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit\\ Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Scale\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Position\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture \\Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter \\ Color\end{tabular}} \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Test \\ Acc.\end{tabular}} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} \\ \hline
 \multicolumn{16}{c}{\textit{State-of-the-Art methods on ResNet-18}}    \\ 
\gls*{ERM}    & 36.5 & 77.7 & 31.8  & 86.8  & 30.9  & 86.8  & 30.9 & 76.0  & 31.9  & 42.1  & 35.8   & 46.9  & 35.2   & 47.2  & 35.3   \\ 
\gls*{UpWt}   & 39.8 & 82.2 & 35.1  & 88.8  & 34.4  & 88.8  & 34.4 & 76.4  & 35.7  & 45.9  & 39.2  &  50.4 & 38.6 & 48.1  & 38.9 \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    & 20.8 & 59.0 & 16.5  & 60.7  & 16.4  & 60.7  & 16.4 & 64.2  & 15.9  & 29.2  & 19.9  & 26.9  & 20.1   & 35.3  & 19.3 \\
\gls*{PGI}~\cite{ahmed2020systematic}    & 49.8 & 85.9 & 45.7  & 94.1  & 44.9 & 94.1 & 44.9 & 79.1  & 46.4 & 54.9  & 49.2  & 68.7  & 47.6  & 55.9  & 49.1 \\
\gls*{SD}~\cite{pezeshki2020gradient}    & &  &   &   &   &   &  &   &   &   &   &   &    &   &   \\ \hline
\multicolumn{16}{c}{\textit{OccamResNet-18 without Input Gating, Exit Gating and Dynamic Pooling}}    \\
\gls*{ERM}     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ 
\gls*{UpWt}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{PGI}~\cite{ahmed2020systematic}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{SD}~\cite{pezeshki2020gradient}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\ \hline
\multicolumn{16}{c}{\textit{Ours: OccamResNet-18 with Input Gating, Exit Gating and Dynamic Pooling}}    \\
Ours     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ \hline
\end{tabular}}
\end{table*}

==> tables/old/biased-mnist-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Results on \gls*{BiasedMNIST}}
\label{tab:biased-mnist}
\addtolength\tabcolsep{1pt}
\begin{tabular}{lcccccccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}l@{}}Unbiased\\Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Digit \\Color\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Digit\\Scale\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Digit\\Position\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Background \\Texture\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Texture\\Color\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Letter\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Letter\\Color\end{tabular} \\\hline
\multicolumn{8}{c}{\textit{ResNet-10 baselines}}                                                             \\
\gls*{ERM}                                                                                              &  &  &  & & & &   \\
\gls*{UpWt}                                                                    &  &  &  & & & &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                               &  &  &  & & & & \\
\gls*{PGI}~\cite{ahmed2020systematic}                                           &  &  &  & & & &   \\
\gls*{SD}~\cite{pezeshki2020gradient}                                                                  &  &  &  & & & &  \\
\hline
\multicolumn{8}{c}{\textit{OccamResNet-10 without Input Gating, Exit Gating and Dynamic Pooling}}                             \\
\gls*{ERM}                                                                                              &  &  &  &  & & &  \\
\gls*{UpWt}                                                                    &  &  &  &  & & &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                               &  &  &  &  & & &  \\
\gls*{PGI}~\cite{ahmed2020systematic}                                           &  &  &  &  & & &  \\ 
\gls*{SD}~\cite{pezeshki2020gradient}                                                                  &  &  &  &  & & &  \\
\hline
\multicolumn{8}{c}{\textit{Ours: OccamResNet-10 with Input Gating, Exit Gating and Dynamic Pooling}}                                                 \\
Full                                                                            &  &  &  &  & & &  \\ \hline
\end{tabular}%
\end{table}

==> tables/old/biased-mnist.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Overall test accuracy (unbiased accuracy) and majority (Maj.)/minority (Min.) accuracies based on each of the bias variables in \gls*{BiasedMNIST} ($p_{bias}=0.95$)}
\label{tab:biased-mnist}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc} \hline
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Variables/\\ Methods\end{tabular}}} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit\\ Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Scale\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Position\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture \\Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter \\ Color\end{tabular}} \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Test \\ Acc.\end{tabular}} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} \\ \hline
 \multicolumn{16}{c}{\textit{State-of-the-Art methods on ResNet-18}}    \\ 
\gls*{ERM}  &  36.7 & 79.9 & 31.8 & 86.9 & 31.1 & 86.9 & 31.1 & 74.1 & 32.4 & 41.9 & 36.1 & 46.8 & 35.5 & 46.1 & 35.7  \\ 
\gls*{UpWt} &  38.2 & 77.2 & 33.8 & 85.7 & 32.9 & 85.7 & 32.9 & 75.3 & 34.0 & 43.7 & 37.6 & 51.3 & 36.7 & 49.9 & 36.9 \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    & 20.8 & 59.0 & 16.5  & 60.7  & 16.4  & 60.7  & 16.4 & 64.2  & 15.9  & 29.2  & 19.9  & 26.9  & 20.1   & 35.3  & 19.3 \\
\gls*{PGI}~\cite{ahmed2020systematic}    & 49.8 & 85.9 & 45.7  & 94.1  & 44.9 & 94.1 & 44.9 & 79.1  & 46.4 & 54.9  & 49.2  & 68.7  & 47.6  & 55.9  & 49.1 \\
\gls*{SD}~\cite{pezeshki2020gradient}    & &  &   &   &   &   &  &   &   &   &   &   &    &   &   \\ \hline
\multicolumn{16}{c}{\textit{OccamResNet-18 without Input Gating, Exit Gating and Dynamic Pooling}}    \\
\gls*{ERM}     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ 
\gls*{UpWt}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{PGI}~\cite{ahmed2020systematic}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{SD}~\cite{pezeshki2020gradient}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\ \hline
\multicolumn{16}{c}{\textit{Ours: OccamResNet-18 with Input Gating, Exit Gating and Dynamic Pooling}}    \\
Ours     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ \hline
\end{tabular}}
\end{table*}

==> tables/old/biased-mnist_0.9.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Unbiased Accuracy (i.e., overall test set accuracy) and Majority/Minority Accuracies per bias variable in \gls*{BiasedMNIST}}
\label{tab:biased-mnist}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc} \hline
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Variables/\\ Methods\end{tabular}}} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit\\ Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Scale\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Position\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture \\Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter \\ Color\end{tabular}} \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Test \\ Acc.\end{tabular}} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} &
  \multicolumn{1}{l}{Maj.} &
  \multicolumn{1}{l}{Min.} \\ \hline
\gls*{ERM}     & 58.7 & 92.4   & 54.9   & 94.9   & 54.7  & 94.9  & 54.7 & 89.6  &  55.3  & 60.1  & 58.6   & 71.0  & 57.3  & 64.4  & 58.1  \\ 
\gls*{UpWt}    & 59.4 & 92.6  & 55.7  & 94.8  & 55.5  & 94.8  & 55.5 & 89.7  & 55.9  & 63.0  & 59.0  & 73.1  & 57.8   & 66.9  & 58.6 \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    & 20.8 & 61.0  & 16.3  & 50.6  & 17.5  & 50.6  & 17.5 & 55.2  & 16.9  & 25.9  & 20.2  & 31.9  & 19.5  &  38.8  & 18.9 \\
\gls*{PGI}~\cite{ahmed2020systematic}    &  71.0 & 95.5  & 68.5  & 96.8  & 68.4  & 96.8  & 68.4 & 93.3  & 68.7  & 73.2  & 70.9  & 81.9  & 69.9  & 73.7  & 70.9 \\
\gls*{SD}~\cite{pezeshki2020gradient}    & 63.7 & 93.7  & 60.3  & 95.4  & 60.1  & 95.4  & 60.1 & 92.8  & 60.4  & 67.4  & 63.2  & 74.4  & 62.4  & 72.2  & 62.7  \\ \hline
\multicolumn{16}{c}{\textit{OccamResNet-10 without Input Gating, Exit Gating and Dynamic Pooling}}    \\
\gls*{ERM}     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ 
\gls*{UpWt}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{PGI}~\cite{ahmed2020systematic}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\
\gls*{SD}~\cite{pezeshki2020gradient}    &  &   &   &   &   &   & &   &   &   &   &   &   &   &  \\ \hline
\multicolumn{16}{c}{\textit{Ours: OccamResNet-10 with Input Gating, Exit Gating and Dynamic Pooling}}    \\
Ours     &  &   &   &   &   &   & &   &   &   &   &   &   &   &   \\ \hline
\end{tabular}}
\end{table*}

==> tables/old/celeba-3-sec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Results on \gls*{CelebA}}
\label{tab:celeba}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}c@{}}Non-Blond\\ Male\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Blond\\Male\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Non-Blond \\ Non-Male \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Blond \\ Non-Male\end{tabular}  &
  \begin{tabular}[c]{@{}c@{}}Mean Per \\ Group\end{tabular} \\ \hline
\multicolumn{6}{c}{\textit{ResNet-18 baselines}}                                                             \\
\gls*{ERM}  & 99.3 & 42.8 & 95.9 & 83.3 & 80.3 \\
\gls*{UpWt}   & 89.3 & 77.8 & 87.4 & 95.0 & 87.4 \\
\gls*{gDRO}~\cite{sagawa2019distributionally} & 91.2 & 80.0 & 90.9 & 92.1 & 88.5 \\
\gls*{PGI}~\cite{ahmed2020systematic}   & 98.2  & 63.3 & 96.5 & 83.9 & 85.5 \\
\gls*{SD}~\cite{pezeshki2020gradient}                                   & 96.4 & 73.3 & 88.0 & 96.6 & 88.6 \\
\hline
\multicolumn{6}{c}{\textit{OccamResNet-18 without Input Gating, Exit Gating and Dynamic Pooling}}                             \\
\gls*{ERM}               & & & & & \\
\gls*{UpWt}   & & & & & \\
\gls*{gDRO}~\cite{sagawa2019distributionally}   & & & & & \\
\gls*{PGI}~\cite{ahmed2020systematic}  & & & & & \\ 
\gls*{SD}~\cite{pezeshki2020gradient}     & & & & & \\\hline
\multicolumn{6}{c}{\textit{Ours: OccamResNet-18 with Input Gating, Exit Gating and Dynamic Pooling}}                                                 \\
OccamResNet-18                                                                            &  &  &  & &  \\ \hline
\end{tabular}%
\end{table}

==> tables/old/coco-on-places-3-sec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Results on \gls*{COCO}}
\label{tab:coco-on-places}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lcccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}c@{}}In-\\ Distribution\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Non-Systematic \\ Shift\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Systematic \\ Shift \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Anomaly \\ Detection\end{tabular} \\ \hline
\multicolumn{5}{c}{\textit{ResNet-18 baselines}}                                                             \\
\gls*{ERM}  & 84.3	& 48.8 & 31.0 & 18.2 \\
\gls*{UpWt}  & 83.2 & 47.6 & 32.7 & 19.6 \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                             & 76.7 & 41.7 & 30.2  & 16.1  \\
\gls*{PGI}~\cite{ahmed2020systematic} & 76.7 &	51.0 &	41.0 &	20.9 \\ 
\gls*{SD}~\cite{pezeshki2020gradient}                                         & 83.9 & 50.3 & 33.4 & 18.2  \\
\hline
\multicolumn{5}{c}{\textit{OccamResNet-18 without Input Gating, Exit Gating and Dynamic Pooling}}                             \\
\gls*{ERM}                                                                                             &  & &	&  \\
\gls*{UpWt}                                                                    & & &		&  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                            & & &	& \\
\gls*{PGI}~\cite{ahmed2020systematic}                                        &  & &	&  \\
\gls*{SD}~\cite{pezeshki2020gradient}                                                                  & & &	 &	 \\\hline
\multicolumn{5}{c}{\textit{Ours: OccamResNet-18 with Input Gating, Exit Gating and Dynamic Pooling}}                                                 \\
OccamResNet-18                                                                            &  &  &  &  \\ \hline
\end{tabular}%
\end{table}

==> tables/old/imagenet-lt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Results on ImageNetLT}
\label{tab:imagenet-lt}
%\resizebox{\textwidth}{!}{%
\addtolength\tabcolsep{5pt}
\begin{tabular}{lcccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}l@{}}Many\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Medium\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Few \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}All\end{tabular} \\ \hline
\multicolumn{5}{c}{\textit{ResNet-50 baselines}}                                                             \\
ERM                                                                                              & 67.6	& 41.1 &	10.6 &	46.9  \\
Up Wt. & 67.3	& 41.5 &	11.1 &	46.9   \\
gDRO~\cite{nam2020learning}   & 60.8 &	37.6 &	12.7 &	42.9  \\
SD~\cite{pezeshki2020gradient} & 67.3 & 41.6 & 11.9  & 47.2  \\
\hline
\multicolumn{5}{c}{\textit{Fair Baseline (3-branched, multi-exit ResNet-50 on RGB images)}}                             \\
ERM                                                                                              &  &  &  &  \\
Up Wt.                                                                    &  &  &  &  \\
gDRO~\cite{DBLP:journals/corr/abs-1911-08731}                                                             &  &  &  &  \\
SD~\cite{pezeshki2020gradient}                                                                  &  &  &  &  \\
\hline
\multicolumn{5}{c}{\textit{Other state-of-the-art methods (published numbers)}}    \\
RIDE (ResNeXt-50)~\cite{wang2020long}                                           & 68.0  & 52.9 & 35.1 & 56.3 \\
TADE (ResNeXt-50)~\cite{zhang2021test}                                           & 67.0  & 56.7 & 42.6 & 58.8 \\\hline

\multicolumn{5}{c}{\textit{OccamResNet-50 (with ablations)}}                                                 \\
OccamResNet-50 (full)                                                                            &  &  &  &  \\
RGB instead of PCA                                                                           &  &  &  &  \\
\begin{tabular}[c]{@{}l@{}}Final exits only\end{tabular}       &  &  &  &  \\
\begin{tabular}[c]{@{}l@{}}Global avg pool\end{tabular} &  &  &  & \\ \hline
\end{tabular}%
%}
\end{table}

==> tables/old/overall-best-3.tex <==
\begin{table}[]
\centering
\caption{Unbiased test set accuracies comparing \gls*{OccamResNet} to the more conventional \gls*{ResNet} architectures without early exits and constrained class activation maps. We format the $\textbf{\underline{first}}$, $\textbf{second}$ and $\underline{third}$ best results. }
\label{tab:overall}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}l@{}}\gls*{BiasedMNIST}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{COCO}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{BAR} \end{tabular} \\ \hline
\multicolumn{4}{c}{\textit{Results on Standard \gls*{ResNet}}}                                                             \\
Base (\gls*{ERM}) (Base)  & 36.8 \tiny{$\pm$ 0.7} & 35.6 \tiny{$\pm$ 1.0}  & 51.3 \tiny{$\pm$1.9}    \\
\gls*{SD}~\cite{pezeshki2020gradient} & 37.1 \tiny{$\pm$ 1.0} & 35.4 \tiny{$\pm$ 0.5}  & 51.3 \tiny{$\pm$2.3}    \\
\gls*{UpWt} & 37.7 \tiny{$\pm$ 1.6} & 35.2 \tiny{$\pm$ 0.4}  & 51.1 \tiny{$\pm$1.9}   \\
\gls*{gDRO}~\cite{sagawa2019distributionally} & 19.2 \tiny{$\pm$ 0.9} & 35.3 \tiny{$\pm 0.1$}  & 38.7 \tiny{$\pm$2.2}  \\
\gls*{PGI}~\cite{ahmed2020systematic} & \underline{48.6} \tiny{$\pm$ 0.7} & \underline{42.7} \tiny{$\pm$ 0.6} & \textbf{53.6} \tiny{$\pm$0.9} \\ 
\hline
\multicolumn{4}{c}{\textit{Results on \gls*{OccamResNet}}}                                                             \\
\gls*{OccamResNet} & \textbf{65.0} \tiny{$\pm 1.0$} & \textbf{43.4} \tiny{$\pm$ 1.0} & \underline{52.6} \tiny{$\pm$1.9} \\
\gls*{OccamResNet}+PGI & \textbf{\underline{69.6}} \tiny{$\pm 0.7$} & \textbf{\underline{43.6}} \tiny{$\pm$ 0.6} & \textbf{\underline{55.9}} \tiny{$\pm$0.7} \\
\hline
\end{tabular}%
\end{table}
% If there is some combination (ours+XXX) does really good, We could separate Ours into two lines, Ours: Occament and Ours:Final (Occamnet+PGI) perhaps...

==> tables/old/overall-single-run.tex <==
\begin{table}[]
\centering
\caption{Unbiased test set accuracies comparing bias mitigation methods on \gls*{ResNet} to \gls*{OccamResNet}.  We format the $\textbf{\underline{first}}$, $\textbf{second}$ and $\underline{third}$ best results.}
\label{tab:overall}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}l@{}}\gls*{BiasedMNIST}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{COCO}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{BAR} \end{tabular} \\ \hline
\multicolumn{4}{c}{\textit{Results on Standard \gls*{ResNet}}}                                                             \\
Base (\gls*{ERM})  & 36.7 & 35.1  & ?    \\
\gls*{SD}~\cite{pezeshki2020gradient} & \underline{38.2} & 35.6  & ?    \\
\gls*{UpWt} & \underline{38.2} & \underline{36.2}  & ?   \\
\gls*{gDRO}~\cite{sagawa2019distributionally} & 20.7 & 32.1  & ?  \\
\gls*{PGI}~\cite{ahmed2020systematic} & \textbf{50.8} & \textbf{42.2} & ? \\ 
\hline
Ours: \gls*{OccamResNet} & \textbf{\underline{66.6}} & \textbf{\underline{43.7}} & ? \\\hline
\end{tabular}%
\end{table}

==> tables/old/overall-with-PGI.tex <==
\begin{table}[]
\centering
\footnotesize
\caption{Unbiased test set accuracies comparing \gls*{OccamResNet} to the more conventional \gls*{ResNet} architectures without early exits and constrained class activation maps. We format the $\textbf{\underline{first}}$, $\textbf{second}$ and $\underline{third}$ best results. }
\label{tab:overall}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccc}
 \hline
Architecture+Method &
  \begin{tabular}[c]{@{}l@{}}\gls*{BiasedMNIST}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{COCO}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{BAR} \end{tabular} \\ \hline
\multicolumn{4}{c}{\textit{Results on Standard \gls*{ResNet}}}                                                             \\
ResNet+ERM  & 36.8 \tiny{$\pm$ 0.7} & 35.6 \tiny{$\pm$ 1.0}  & 51.3 \tiny{$\pm$1.9}    \\
ResNet+\gls*{SD}~\cite{pezeshki2020gradient} & 37.1 \tiny{$\pm$ 1.0} & 35.4 \tiny{$\pm$ 0.5}  & 51.3 \tiny{$\pm$2.3}    \\
ResNet+\gls*{UpWt} & 37.7 \tiny{$\pm$ 1.6} & 35.2 \tiny{$\pm$ 0.4}  & 51.1 \tiny{$\pm$1.9}   \\
ResNet+\gls*{gDRO}~\cite{sagawa2019distributionally} & 19.2 \tiny{$\pm$ 0.9} & 35.3 \tiny{$\pm 0.1$}  & 38.7 \tiny{$\pm$2.2}  \\
ResNet+\gls*{PGI}~\cite{ahmed2020systematic} & \underline{48.6} \tiny{$\pm$ 0.7} & \underline{42.7} \tiny{$\pm$ 0.6} & \textbf{53.6} \tiny{$\pm$0.9} \\ 
\hline
\multicolumn{4}{c}{\textit{Results on \gls*{OccamResNet}}}                                                             \\
\gls*{OccamResNet} & \textbf{65.0} \tiny{$\pm 1.0$} & \textbf{43.4} \tiny{$\pm$ 1.0} & \underline{52.6} \tiny{$\pm$1.9} \\
\gls*{OccamResNet}+PGI & \textbf{\underline{69.6}} \tiny{$\pm 0.7$} & \textbf{\underline{43.6}} \tiny{$\pm$ 0.6} & \textbf{\underline{55.9}} \tiny{$\pm$0.7} \\
\hline
\end{tabular}%
\end{table}
% If there is some combination (ours+XXX) does really good, We could separate Ours into two lines, Ours: Occament and Ours:Final (Occamnet+PGI) perhaps...

==> tables/old/position-bias-included-biased-mnist.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Overall test accuracy (unbiased accuracy) and majority (Maj)/minority (Min) accuracies on each of the bias variables in \gls*{BiasedMNIST} ($p_{bias}=0.95$)}
\label{tab:biased-mnist}
\addtolength\tabcolsep{1.75pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc} \hline
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Variables/\\ Methods\end{tabular}}} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit\\ Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Scale\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Digit \\ Position\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Texture \\Color\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Letter \\ Color\end{tabular}} \\
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Test \\ Acc.\end{tabular}} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min} &
  \multicolumn{2}{c}{Maj/Min}
  \\ \hline
 \multicolumn{16}{c}{\textit{Comparison Methods on ResNet18}}    \\ 
 \multicolumn{1}{l}{Base (\gls*{ERM})} &
  \multicolumn{1}{l}{36.8} &
  \multicolumn{2}{c}{78.5/32.1} &
  \multicolumn{2}{c}{87.2/31.3} &
  \multicolumn{2}{c}{87.2/31.3} &
  \multicolumn{2}{c}{76.1/32.4} &
  \multicolumn{2}{c}{41.9/36.3} &
  \multicolumn{2}{c}{46.7/35.7} &
  \multicolumn{2}{c}{45.7/35.9}
  \\
  \multicolumn{1}{l}{\gls*{SD}~\cite{pezeshki2020gradient}} &
  \multicolumn{1}{l}{37.1} &
  \multicolumn{2}{c}{76.9/32.7} &
  \multicolumn{2}{c}{83.4/32.0} &
  \multicolumn{2}{c}{83.4/32.0} &
  \multicolumn{2}{c}{76.7/32.7} &
  \multicolumn{2}{c}{42.3/36.6} &
  \multicolumn{2}{c}{48.3/35.8} &
  \multicolumn{2}{c}{48.9/35.9}
  \\
  \multicolumn{1}{l}{\gls*{UpWt}} &
  \multicolumn{1}{l}{37.7} &
  \multicolumn{2}{c}{80.4/32.9} &
  \multicolumn{2}{c}{88.0/32.1} &
  \multicolumn{2}{c}{88.0/32.1} &
  \multicolumn{2}{c}{75.6/33.4} &
  \multicolumn{2}{c}{41.9/37.2} &
  \multicolumn{2}{c}{46.7/36.6} &
  \multicolumn{2}{c}{46.9/36.7}
  \\
  \multicolumn{1}{l}{\gls*{gDRO}~\cite{sagawa2019distributionally}} &
  \multicolumn{1}{l}{19.2} &
  \multicolumn{2}{c}{50.2/15.7} &
  \multicolumn{2}{c}{55.0/15.2} &
  \multicolumn{2}{c}{55.0/15.2} &
  \multicolumn{2}{c}{63.4/14.2} &
  \multicolumn{2}{c}{24.8/18.6} &
  \multicolumn{2}{c}{26.7/18.3} &
  \multicolumn{2}{c}{29.5/18.1}
  \\
  \multicolumn{1}{l}{\gls*{PGI}~\cite{ahmed2020systematic}} &
  \multicolumn{1}{l}{48.6} &
  \multicolumn{2}{c}{84.8/44.6} &
  \multicolumn{2}{c}{91.9/43.8} &
  \multicolumn{2}{c}{91.9/43.8} &
  \multicolumn{2}{c}{79.5/45.1} &
  \multicolumn{2}{c}{51.3/48.3} &
  \multicolumn{2}{c}{67.2/46.5} &
  \multicolumn{2}{c}{55.8/47.9}
  \\ \hline
  \multicolumn{16}{c}{\textit{Comparison Methods on \gls*{OccamResNet}18} with all the proposed losses}    \\ 
   \multicolumn{1}{l}{Base (Occam)} &
  \multicolumn{1}{l}{\underline{65.0}} &
  \multicolumn{2}{c}{96.3/61.5} &
  \multicolumn{2}{c}{94.6/61.7} &
  \multicolumn{2}{c}{94.6/61.7} &
  \multicolumn{2}{c}{81.6/63.1} &
  \multicolumn{2}{c}{66.8/64.8} &
  \multicolumn{2}{c}{64.7/65.1} &
  \multicolumn{2}{c}{64.7/65.1}
  \\
  \multicolumn{1}{l}{\gls*{SD}~\cite{pezeshki2020gradient}} &
  \multicolumn{1}{l}{55.2} &
  \multicolumn{2}{c}{92.9/50.9} &
  \multicolumn{2}{c}{92.3/51.1} &
  \multicolumn{2}{c}{92.3/51.1} &
  \multicolumn{2}{c}{78.9/52.5} &
  \multicolumn{2}{c}{57.4/54.9} &
  \multicolumn{2}{c}{55.9/55.1} &
  \multicolumn{2}{c}{55.3/55.2}
  \\
    \multicolumn{1}{l}{\gls*{UpWt}} &
  \multicolumn{1}{l}{\textbf{65.7}} &
  \multicolumn{2}{c}{96.3/62.3} &
  \multicolumn{2}{c}{95.1/62.5} &
  \multicolumn{2}{c}{95.1/62.5} &
  \multicolumn{2}{c}{82.4/63.9} &
  \multicolumn{2}{c}{68.3/65.5} &
  \multicolumn{2}{c}{65.3/65.8} &
  \multicolumn{2}{c}{65.3/65.8}
  \\
  \multicolumn{1}{l}{\gls*{gDRO}~\cite{sagawa2019distributionally}} &
  \multicolumn{1}{l}{29.8} &
  \multicolumn{2}{c}{69.5/25.3} &
  \multicolumn{2}{c}{72.8/25.0} &
  \multicolumn{2}{c}{72.8/25.0} &
  \multicolumn{2}{c}{45.8/28.0} &
  \multicolumn{2}{c}{39.4/28.8} &
  \multicolumn{2}{c}{29.7/29.8} &
  \multicolumn{2}{c}{36.1/29.1}
  \\
   \multicolumn{1}{l}{\gls*{PGI}~\cite{ahmed2020systematic}} &
  \multicolumn{1}{l}{\textbf{\underline{69.6}}} &
  \multicolumn{2}{c}{97.0/66.5} &
  \multicolumn{2}{c}{95.4/66.7} &
  \multicolumn{2}{c}{95.4/66.7} &
  \multicolumn{2}{c}{88.6/67.4} &
  \multicolumn{2}{c}{71.4/69.4} &
  \multicolumn{2}{c}{69.6/69.6} &
  \multicolumn{2}{c}{70.5/69.5}
  \\ \hline

\end{tabular}}
\end{table*}

==> tables/old/row-wise-overall.tex <==
\begin{table}[]
\centering
\caption{Comparisons}
\label{tab:overall}
\addtolength\tabcolsep{5pt}
\begin{tabular}{lccc}
 \hline
Methods &
  \begin{tabular}[c]{@{}l@{}}\gls*{BiasedMNIST}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{COCO}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\gls*{CelebA} \end{tabular} \\ \hline
\multicolumn{4}{c}{\textit{Standard \gls*{ResNet}}}                                                             \\
Base (\gls*{ERM})                                                                                              &  & 31.0  & 80.3    \\ \hline
\multicolumn{4}{c}{\textit{State-of-the-Art Methods on Standard ResNet}}                             \\\hline
\gls*{SD}~\cite{pezeshki2020gradient}                                                                  &  & 33.4  & 88.6    \\
\gls*{UpWt}                                                                   & & 32.7  & 87.4   \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                               &  & 30.2  & 88.5  \\
\gls*{PGI}~\cite{ahmed2020systematic}                                           &  & 41.0 & 85.5 \\ 
\\\hline \hline
\multicolumn{4}{c}{\textit{\gls*{OccamResNet}}}                             \\
Ours: \gls*{OccamResNet}                                                                                            &  &  &  \\\hline
\multicolumn{4}{c}{\textit{State-of-the-Art Methods on Occam ResNet}}                             \\
\gls*{SD}~\cite{pezeshki2020gradient}                                                                  &  &  &  \\

\gls*{UpWt}                                                                    &  &  &  \\
\gls*{gDRO}~\cite{sagawa2019distributionally}                                                               &  &  &  \\
\gls*{PGI}~\cite{ahmed2020systematic}                                           &  &  &  \\ \hline
\end{tabular}%
\end{table}

==> tables/old/two-col-resnet-vs-occam-resnet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{ResNet versus OccamResNet unbiased accuracies on all the datasets and methods.}
\label{tab:overall-std-vs-occam}
\addtolength\tabcolsep{3pt}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllll}
\hline
 &
  \multicolumn{2}{c}{\gls*{BiasedMNIST}} &
  \multicolumn{2}{c}{\gls*{COCO}} &
  \multicolumn{2}{c}{\gls*{BAR}} \\ \hline
 \begin{tabular}[l]{@{}l@{}}Architectures /\\ Methods\end{tabular} &
  ResNet &
  \begin{tabular}[l]{@{}l@{}}Occam-\\ ResNet\end{tabular} &
  ResNet &
  \begin{tabular}[l]{@{}l@{}}Occam-\\ ResNet\end{tabular} &
  ResNet &
  \begin{tabular}[l]{@{}l@{}}Occam-\\ ResNet\end{tabular} \\ \hline
Base & 36.8 \tiny{$\pm$ 0.7}  & \textbf{65.0} \tiny{$\pm$ 1.0} & 35.6 \tiny{$\pm$ 1.0}  & \textbf{43.4} \tiny{$\pm$ 1.0}  & 51.3 \tiny{$\pm$1.9} & \underline{52.6} \tiny{$\pm$1.9} \\
\gls*{SD}~\cite{pezeshki2020gradient}   & 37.1 \tiny{$\pm$1.0} & 55.2 \tiny{$\pm$ 3.8}  & 35.4 \tiny{$\pm$ 0.5} & 39.4 \tiny{$\pm$ 0.6} & 51.3\tiny{$\pm$2.3} & 52.3 \tiny{$\pm$2.4} \\
\gls*{UpWt} & 37.7 \tiny{$\pm$} 1.6 & \underline{65.7} \tiny{$\pm$}2.6 & 35.2 \tiny{$\pm$ 0.4} & \underline{42.9} \tiny{$\pm$ 0.8} & 51.1 \tiny{$\pm$1.9} & 52.2 \tiny{$\pm$1.4} \\
\gls*{gDRO}~\cite{sagawa2019distributionally} & 19.2 \tiny{$\pm$ 0.9}  & 29.8 \tiny{$\pm$ 2.5}  & 35.3 \tiny{$\pm$ 0.1} & 40.7 \tiny{$\pm$ 1.5} & 38.7 \tiny{$\pm$2.2} & \textbf{52.9} \tiny{$\pm$0.8} \\
\gls*{PGI}~\cite{ahmed2020systematic} & 48.6 \tiny{$\pm$ 0.7} & \textbf{\underline{69.6}} \tiny{$\pm$ 0.7} & 42.7 \tiny{$\pm$ 0.6} & \textbf{\underline{43.6}} \tiny{$\pm$ 0.6} & \textbf{\underline{53.6}} \tiny{$\pm$0.9} & 52.5 \tiny{$\pm$ 3.4} \\ \hline
\end{tabular}%
%}
\end{table}
